HybriMoE: Hybrid CPU-GPU Scheduling and Cache Management for Efficient MoE Inference

The Mixture of Experts (MoE) architecture has demonstrated significant advantages as it enables to increase the model capacity without a proportional increase in computation. However, the large MoE model size still introduces substantial memory demands, which usually requires expert offloading on resource-constrained platforms and incurs significant overhead. Hybrid CPU-GPU inference has been proposed to leverage CPU computation to reduce expert loading overhead but faces major challenges: on one hand, the expert activation patterns of MoE models are highly unstable, rendering the fixed mapping strategies in existing works inefficient; on the other hand, the hybrid CPU-GPU schedule for MoE is inherently complex due to the diverse expert sizes, structures, uneven workload distribution, etc. To address these challenges, in this paper, we propose HybriMoE, a hybrid CPU-GPU inference framework that improves resource utilization through a novel CPU-GPU scheduling and cache management system. HybriMoE introduces (i) a dynamic intra-layer scheduling strategy to balance workloads across CPU and GPU, (ii) an impact-driven inter-layer prefetching algorithm, and (iii) a score-based caching algorithm to mitigate expert activation instability. We implement HybriMoE on top of the kTransformers framework and evaluate it on three widely used MoE-based LLMs. Experimental results demonstrate that HybriMoE achieves an average speedup of 1.33$\times$ in the prefill stage and 1.70$\times$ in the decode stage compared to state-of-the-art hybrid MoE inference framework. Our code is available at: https://github.com/PKU-SEC-Lab/HybriMoE.

==> docs/outline.tex <==
\section*{Outline}
\begin{itemize}
    \item \textbf{MoE offloading background.} Despite the training efficiency and computational benefits, MoE models face deployment challenges in memory-limited environments, particularly on edge devices. Offloading expert weights to CPU memory, SSDs, or other storage can mitigate memory constraints but often leads to high latency due to on-demand loading, especially when expert selection and execution occur sequentially. 

    \item \textbf{CPU-GPU background.} On modern edge devices, CPUs and GPUs work together, each specializing in different tasks. While GPUs excel in large-scale parallel computation, they have limited cache capacity and are constrained in data loading. CPUs, on the other hand, offer greater flexibility in managing cache and can compensate for GPU load during cache miss
    \item \textbf{Existing solutions and their limitations.} Several existing methods have explored caching and scheduling optimizations for MoE models within a heterogeneous CPU-GPU environment, but these approaches have notable limitation
        \begin{itemize}  
            \item \textbf{Powerinfer} focuses on neuron-level sparsity and is effective when activation frequencies vary widely. However, it lacks the capability to manage expert-level sparsity effectively, whose activation frequency variation is smaller.
            \item \textbf{Fiddler} and \textbf{Ktransformers} implements CPU-GPU co-optimization to reduce data transfer. However, they adopt a fixed expert mapping method, ignoring the complex situations under different \textbf{workload} intensity of \textbf{experts} and \textbf{devices}.
            \begin{itemize}
                \item Expert workload: The workload of activated experts may be different in prefill stage and multi-batch decode stage.
                \item Device workload: The cache hit situation of GPU varies under different inputs.
            \end{itemize}
        \end{itemize}
    \item \textbf{Opportunities.} ProMoE, AdapMoE and Hobbit propose specialized prefetching and caching to relieve the on-demand loading overhead. These mechanisms can better balance the workload between CPU and GPU.
    \item \textbf{Key challenges in Heterogeneous Edge MoE inference}
        \begin{itemize}
            \item \textbf{Complexity of Heterogeneous Scheduling.} There is a significant variance in the computation workload of different experts and devices(CPU-GPU), especially in multi-batch MoE inference. Effective heterogeneous scheduling requires intelligent task distribution, where high-load experts are allocated to GPUs, while some tasks are dynamically offloaded to CPUs when GPU resources are constrained, balancing the load and optimizing overall inference efficiency.
            \begin{itemize}
                \item Huge workload allocation search space.
                \item The execution time \textbf{does not increase linearly} with workload quantity.
            \end{itemize}
            \item \textbf{Complexity of MoE-Specific Cache and Prefetch Strategies.} Integrating cache and prefetch strategies with MoE’s dynamic expert activation patterns and CPU-GPU heterogeneous scheduling presents a unique challenge. Effective solutions must adapt to MoE’s sparse activation, prioritizing high-demand experts in multi-batch settings while dynamically coordinating task allocation across CPU and GPU resources.
            \item difference between mixtral and other moe models, and different kernels, hardware capabilities
        \end{itemize}
    \item Main Contributions
        \begin{itemize}
            \item \textbf{Hybrid CPU-GPU Task Scheduling:} A novel scheduling strategy that dynamically allocates high-load experts to GPU processing while leveraging CPU resources for non-critical tasks during cache misses.
            \item \textbf{MoE-speciliazed Cache Management:} An expert score-based caching strategy that prioritizes high-demand experts across layers, especially under multi-batch conditions, to minimize cache misses.
            \item \textbf{System-Aware Prefetching Strategy:} A prefetching mechanism that considers both cache status and CPU-GPU resource availability, dynamically adjusting prefetch targets to maximize resource utilization across layers.
        \end{itemize}
    \item Experiments
        \begin{itemize}
            \item End-to-End performance, totally 9 figures
                \begin{itemize}
                    \item Different cache size(in 1 figure)
                    \item Different models(Mixtral, DeepSeek, Qwen2)
                    \item Different batch size(1,2,4)
                \end{itemize}
            \item Ablation Study
            \item Score-aware cache management performance
            \item Sensitivity-analysis when the performance of CPU, GPU and CPU-GPU bandwidth change
        \end{itemize}
\end{itemize}


